On the Pseudo-Mixing of Kac's Walk

Motivated by a conjecture of Vaikuntanathan and Zamir, we study the pseudo-mixing of Kac's walk on $\mathrm{SO}(n)$: whether short trajectories are indistinguishable from Haar measure by low-complexity tests. We prove that the first $k$ columns mix in Wasserstein distance in $O(n(k+\log n)\log n)$ steps for fixed accuracy, resolving a conjecture of Oliveira. Combining this with a representation-theoretic variance bound, we show that if $T=\omega(nk(k+\log n)\log n)$, then every degree-$k$ polynomial normalized to have unit Haar variance has expectation under the $T$-step law within $o(1)$ of its Haar expectation. As an application, we show that this pseudo-mixing estimate can be used to prove the effectiveness of a fast Johnson--Lindenstrauss transform with the usual target dimension.

==> macros.tex <==
\usepackage[utf8]{inputenc}
\usepackage{color}
\usepackage{amssymb}
\usepackage{tikz}
\usepackage{subcaption}
\usepackage{caption}
\usepackage{comment}
\usepackage{pdfpages}
\usepackage{soul}
\usepackage{graphicx}% Include figure files
\usepackage{dcolumn}% Align table columns on decimal point
%\setlength\textheight{7.7in}

%\setlength\textwidth{6.5in}
%\setlength\oddsidemargin{0in}
%\setlength\evensidemargin{0in}
%\setlength\parindent{0.25in}
%\setlength\marginparwidth{0.8in}
\usepackage{xcolor}

%\documentclass[aos,preprint,reqno]{imsart}
%\setattribute{journal}{name}{}
\RequirePackage[numbers]{natbib}
\RequirePackage[colorlinks=true, pdfstartview=FitV, linkcolor=blue,
  citecolor=blue, urlcolor=blue, pagebackref]{hyperref}
\usepackage{backref}
\RequirePackage{hypernat}
\usepackage{paralist}


% Vinod's favorite font --- but I know not everyone's in love with it, so feel free to comment it out
\usepackage[utf8]{inputenc}
\usepackage{microtype}      % microtypography
\usepackage{libertine}
\usepackage{libertinust1math}


\newcommand{\cK}{{\mathcal {K}}}
\newcommand{\cL}{{\mathcal {L}}}
\newcommand{\cC}{{\mathcal {C}}}
\def \Sym \mathrm{Sym}
\newcommand{\Tr}{\mathrm{Trace}}
\newcommand{\GD}{E}
\newcommand{\SGD}{E}
\newcommand{\goedist}{KILLTHISNOTATION}
\newcommand{\Ev}{\mathrm{Ev}}
\newcommand{\End}{\mathrm{End}}
\newcommand{\kacdist}{\beta}
\newcommand{\haarOdist}{\alpha}
\newcommand{\GS}{E^{\ast}}
\newcommand{\Ig}{Z_{\mathrm{sub}}}
\newcommand{\Var}{Var}
\newcommand{\supp}{supp}
\newcommand{\TT}{\Theta \times \mathbb{A}}
\newcommand{\So}[1]{\mathcal{SO}(#1)}

%\usepackage{showkeys}
\usepackage{graphicx}
\graphicspath{{./figures/}}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{amsbsy}
\usepackage{epsfig}
\usepackage{fullpage}
\usepackage{natbib, mathrsfs}

\usepackage{verbatim}
%\usepackage[latin1]{inputenc}
\usepackage{mhequ}
\usepackage{algorithm}
%\usepackage{algorithmicx}
\usepackage{algorithmic}
%\usepackage{algpseudocode}
\usepackage[letterpaper,left=1.5in,right=1.5in]{geometry}
\usepackage{enumitem}

% Define keyword and construction of \RETURN
% Come back to this?
%\algnewcommand\RETURN{\State \algorithmicreturn}%
%\usepackage{showlabels}
\numberwithin{equation}{section}


% put your definitions there:
%\startlocaldefs
\def \be{\begin{equs}} 
\def \ee{\end{equs}}
\def \P{\mathbb{P}}
\def \E{\mathbb{E}}
\def \He{\mathfrak{H}}
\newcommand \tv[1]{\|#1\|_{\mathrm{TV}}}
%\newcommand \TV{\mathrm{TV}}

\def \id{\mathrm{id}}
\def \tmix{\tau_{\mathrm{mix}}}
\def \tmixR{\tau_{\mathrm{mix}}^{\mathrm{RW}}}
\def \Z{\mathbb{Z}}
\def \i{\mathbf{i}}
\newcommand \mt[1]{\marginpar{\textcolor{red}{#1}}}
\def \lip{\mathrm{Lip}}
%\def \TV{\mathrm{TV}}
\def \var{\mathrm{Var}}
\def \H{\mathcal{H}}
\def \O{\mathrm{Occ}}
\def \sn{\mathrm{S}^{n-1}}
\def \F{\mathrm{F}}
\newcommand{\tRe}{\tau_{\mathrm{ret}}}
\newcommand{\vmax}{V_{\mathrm{max}}}
\newcommand{\tEsc[1]}{\tau_{#1,\mathrm{esc}}}
\def \S{\mathrm{S}}
\def \prg{\tcr{[FIX ME]}}
\def \FC{Z^{(1)}}
\def \SC{Z^{(2)}}

\def \Tr{\mathrm{Trace}}
\def \SO{\mathrm{SO}}
\def \R{\mathbb{R}}
\def \C{\mathbb{C}}
\def \HS{\mathrm{HS}}

% Trying to fix notation conflicts
\newcommand \Lbtw[4]{L_{btw}(#1, #2,#3,#4)}
\newcommand \Lin[4]{L_{in}(#1, #2,#3,#4)}

\newcommand \Mbtw[5]{M_{btw}^{(#1)}(#2, #3,#4,#5)}
\newcommand \Min[5]{M_{in}^{(#1)}(#2, #3,#4,#5)}

\newcommand \Dbtw[6]{M_{btw}^{(#1)}(#2, #3,#4,#5)}
\newcommand \Din[5]{M_{in}^{(#1)}(#2, #3,#4,#5)}


\newtheorem{theorem}{Theorem}[section]

\newtheorem*{theoremnonum}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{remark}[theorem]{Remark}
%\newtheorem{remarks}[theorem]{Remarks}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{prop}[theorem]{Proposition}
\newtheorem{assumptions}[theorem]{Assumptions}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{heuristic}[theorem]{Heuristic}
\newtheorem{cond}[theorem]{Condition}


\theoremstyle{plain}
\newtheorem{thm}{Theorem}
\newtheorem*{thm-non}{Theorem}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{conj}[thm]{Conjecture}
\newtheorem{heur}[thm]{Heuristic}


\theoremstyle{definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{defn}[theorem]{Definition}
\newtheorem{remark}[theorem]{Remark}
% provide arXiv number if available:
%\arxiv{math.PR/0000000}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% EDITING HELPER FUNCTIONS  %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% NA: needs attention (rough writing whose correctness needs to be verified)
%% TBD: instructions for how to fix a gap (''Describe the propagation by ...'')
%% PROBLEM: bug or missing crucial bit

%% use \fXXX versions of these macros to put additional explanation into a footnote.
%% The idea is that we don't want to interrupt the flow of the paper or make it
%% impossible to read because there are a bunch of comments.

%% NA's (and TBDs, those less crucially) should be written so
%% that they flow with the text.

\definecolor{WowColor}{rgb}{.75,0,.75}
\definecolor{SubtleColor}{rgb}{0.9,0,0}

% inline
\newcommand{\NA}[1]{\textcolor{SubtleColor}{ {\tiny \bf ($\star$)} #1}}
\newcommand{\LATER}[1]{\textcolor{SubtleColor}{ {\tiny \bf ($\dagger$)} #1}}
\newcommand{\TBD}[1]{\textcolor{SubtleColor}{ {\tiny \bf (!)} #1}}
\newcommand{\PROBLEM}[1]{\textcolor{WowColor}{ {\bf (!!)} {#1}}}

% as margin notes

\newcounter{margincounter}
\newcommand{\displaycounter}{{\arabic{margincounter}}}
\newcommand{\incdisplaycounter}{{\stepcounter{margincounter}\arabic{margincounter}}}

\newcommand{\fTBD}[1]{\textcolor{SubtleColor}{$\,^{(\incdisplaycounter)}$}\marginpar{\tiny\textcolor{SubtleColor}{ {\tiny $(\displaycounter)$} #1}}}

\newcommand{\fPROBLEM}[1]{\textcolor{WowColor}{$\,^{((\incdisplaycounter))}$}\marginpar{\tiny\textcolor{WowColor}{ {\bf $\mathbf{((\displaycounter))}$} {\bf #1}}}}


\newcounter{latercounter}
\newcommand{\inclatercounter}{{\stepcounter{latercounter}\arabic{latercounter}}}
\newcommand{\displaylatercounter}{{\arabic{latercounter}}}
\newcommand{\fLATER}[1]{\textcolor{SubtleColor}{$\,^{(\inclatercounter\dagger)}$}\marginpar{\tiny\textcolor{SubtleColor}{ {\tiny $(\displaylatercounter\dagger)$} #1}}}


\ifsub
\newcommand{\authnote}[3]{}
\else
\newcommand{\authnote}[3]{\textcolor{#3}{[{#2}: #1]}}
\fi 
\newcommand{\anote}[1]{\authnote{#1}{AMS}{red}}
\newcommand{\amsnote}[1]{\authnote{#1}{AMS}{red}}
\newcommand{\vnote}[1]{\authnote{#1}{Vinod}{blue}}
\newcommand{\nnote}[1]{\authnote{#1}{Natesh}{green}}
